Addressing Sample Complexity in Visual Tasks Using HER and Hallucinatory GANs

Reinforcement Learning (RL) algorithms typically require millions of environment interactions to learn successful policies in sparse reward settings. Hindsight Experience Replay (HER) was introduced as a technique to increase sample efficiency by reimagining unsuccessful trajectories as successful ones by altering the originally intended goals. However, it cannot be directly applied to visual environments where goal states are often characterized by the presence of distinct visual features. In this work, we show how visual trajectories can be hallucinated to appear successful by altering agent observations using a generative model trained on relatively few snapshots of the goal. We then use this model in combination with HER to train RL agents in visual settings. We validate our approach on 3D navigation tasks and a simulated robotics application and show marked improvement over baselines derived from previous work.

==> images/s-architechtures.tex <==
\section{Network Architectures}
Refer to table below for details on the network architecture for DDQN. LeakyReLu's were used as activations throughout except for the output layer where no activation was used.
\begin{table}[h]
\label{tab:arch-ddqn}
\begin{center}
\begin{small}
\begin{sc}
% \tabcolsep=0.05cm
\begin{tabular}{lccc}
\toprule
Layer & Shape & Filters & \#params\\
\midrule
Image Input & 64x64 & 3 & 0 \\
Conv 1 & 5x5 & 4 &  304\\
Conv 2 & 5x5 & 8 & 808 \\
Conv 3 & 5x5 & 16 & 3216 \\
Conv 4 & 5x5 & 32 & 12832 \\
Dense 1 & 32 & - & 16416\\
Dense 2 & 4 ($nbactions$) & - & 132\\
Total & - & - & 33708 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\caption{Network Architecture for DDQN Agent}
\end{center}
\end{table}


Refer to table below for details on the network architecture for actor for DDPG. LeakyReLu's were used as activations throughout except for the output layer where a Tanh was used.
\begin{table}[h]
\label{tab:arch-ddpg-actor}
\begin{center}
\begin{small}
\begin{sc}
% \tabcolsep=0.05cm
\begin{tabular}{lccc}
\toprule
Layer & Shape & Filters & \#params\\
\midrule
Image Input & 64x64 & 3 & 0 \\
Conv 1 & 5x5 & 4 &  304\\
Conv 2 & 5x5 & 8 & 808 \\
Conv 3 & 5x5 & 16 & 3216 \\
Conv 4 & 5x5 & 32 & 12832 \\
Dense 1 & 32 & - & 16416\\
Dense 2 & 2 ($nbactions$) & - & 66\\
Total & - & - & 33642 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\caption{Network Architecture for DDPG Actor}
\end{center}
\end{table}

Refer to table below for details on the network architecture for critic for DDPG. LeakyReLu's were used as activations throughout except for the output layer where no activation was used.
\begin{table}[h]
\label{tab:arch-ddpg-critic}
\begin{center}
\begin{small}
\begin{sc}
% \tabcolsep=0.05cm
\begin{tabular}{lccc}
\toprule
Layer & Shape & Filters & \#params\\
\midrule
Image Input & 64x64 & 3 & 0 \\
Conv 1 & 5x5 & 4 &  304\\
Conv 2 & 5x5 & 8 & 808 \\
Conv 3 & 5x5 & 16 & 3216 \\
Conv 4 & 5x5 & 32 & 12832 \\
Dense 1 & 32 & - & 16416\\
Dense 2 & 1 & - & 33\\
Total & - & - & 33673 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\caption{Network Architecture for DDPG Critic}
\end{center}
\end{table}

Refer to table below for details on the network architecture for the generator in HALGAN. LeakyReLu's were used as activations throughout except immediately after the conditioning layer where no activation was used and the output where tanh was used.
\begin{table}[h]
\label{tab:arch-halgan-g}
\begin{center}
\begin{small}
\begin{sc}
% \tabcolsep=0.05cm
\begin{tabular}{lccc}
\toprule
Layer & Shape & Filters & \#params\\
\midrule
Config Input & 3 & - & 0 \\
Dense 1 & 128 & - & 384 \\
Conditioning Input & 128 & - &  0\\
Multiply & 128 & - & 0 \\
Reshape & 1x1 & 128 & 0 \\
UpSample + Conv 1 & 4x4 & 64 & 131136 \\
BatchNorm & 2x2 & 64 & 256\\
UpSample + Conv 2 & 4x4 & 64 & 65600 \\
BatchNorm & 4x4 & 64 & 256\\
UpSample + Conv 3 & 4x4 & 64 & 65600 \\
BatchNorm & 8x8 & 64 & 256\\
UpSample + Conv 4 & 4x4 & 32 & 32800 \\
BatchNorm & 16x16 & 32 & 256\\
UpSample + Conv 5 & 4x4 & 32 & 16416 \\
BatchNorm & 32x32 & 32 & 128\\
UpSample + Conv 6 & 4x4 & 16 & 8028 \\
BatchNorm & 64x64 & 16 & 64\\
Conv 7 & 4x4 & 8 & 2056 \\
BatchNorm & 64x64 & 8 & 32\\
Conv 8 & 4x4 & 3 & 387 \\
Total & - & - & 323707 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\caption{Network Architecture HALGAN Generator}
\end{center}
\end{table}

Refer to table below for details on the network architecture for the discriminator in HALGAN. LeakyReLu's were used as activations throughout except at the output where no activation was used.
\begin{table}[h]
\label{tab:arch-halgan-d}
\begin{center}
\begin{small}
\begin{sc}
% \tabcolsep=0.05cm
\begin{tabular}{lccc}
\toprule
Layer & Shape & Filters & \#params\\
\midrule
Image Input & 64x64 & 3 & 0 \\
Conv 1 & 4x4 & 32 &  1568\\
Conv 2 & 4x4 & 32 & 16416 \\
Conv 3 & 4x4 & 32 & 16416 \\
Conv 4 & 4x4 & 64 & 32832 \\
Conv 5 & 4x4 & 64 & 65600 \\
Conv 6 & 4x4 & 64 & 65600 \\
Conv 7 & 4x4 & 128 & 131200 \\
Dense (Aux) & 2 & - & 129\\
Dense (real/fake) & 1: & - & 258\\
Total & - & - & 330019 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\caption{Network Architecture for HALGAN Discriminator}
\end{center}
\end{table}

==> images/s-hyperparameters.tex <==
\section{Experimental Hyperparameters}
Refer to table below for environment specific hyperparameters.
\begin{table}[h]
\label{tab:hyper-experiments}
\begin{center}
\begin{small}
\begin{sc}
% \tabcolsep=0.05cm
\begin{tabular}{lccc}
\toprule
Hyperparameter & TurtleBot & MiniWorld Navigate & MiniWorld Pick-and-Place\\
\midrule
Replay Warmup & 10,000 & 10,000 & 10,000 \\
Replay Capacity & 100,000 & 100,000 & 100,000 \\
Initial Exploration $\epsilon$ & 1.0 & 1.0 & 1.0 \\
Final Exploration $\epsilon$ & 0.5 & 0.5 & 0.5 \\
$\epsilon$ Anneal Steps & 100,000 & 100,000 & 250,000 \\
Discount ($\gamma$) & 0.99 & 0.99 & 0.99 \\
Off-Policy Algorithm & DDQN & DDPG & DDPG \\
Policy Optimizer & ADAM & ADAM & ADAM \\
Learning Rate & $1e^{-3}$ & $1e^{-5}$ (Actor), $1e^{-4}$ (Critic) & $1e^{-5}$ (Actor), $1e^{-4}$ (Critic) \\
Size of $R$ for HALGAN & 6,840 & 2,000 & 6,419 \\
Hallucination Start \% & 20\% & 30\% & 30\% \\ 
Hallucination END \% & 0\% & 0\% & 0\% \\ 
Max Failed Trajectory Length & 16 & 32 & 16 \\
Image size & 64x64 & 64x64 & 64x64 \\
Random Seeds & 75839, 69045, 47040 & 75839, 69045, 47040, & 75839, 69045, 47040, \\
& & 60489, 11798 & 60489, 11798 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\caption{Environment Specific Hyperparameters}
\end{center}
\end{table}

Refer to table below for HALGAN specific hyperparameters.
\begin{table}[h]
\label{tab:hyper-gan}
\begin{center}
\begin{small}
\begin{sc}
% \tabcolsep=0.05cm
\begin{tabular}{lccc}
\toprule
Hyperparameter & Value\\
\midrule
Latent Vector Size & 128 \\
Latent Sampling Distribution & $\mathcal{N}(1,0.1)$ \\
Auxiliary Task Weight & 10 \\
Gradient Penalty Weight & 10 \\
$L_2$ loss on $H$ Weight & 1\\
Optimizer & ADAM \\
Learning Rate & $1e-4$ \\
Adam $\beta1$ & 0.5 \\
Adam $\beta2$ & 0.9 \\
$D$ Iters per $H$ Iter & 5 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\caption{Hyperparameters involved in training HALGAN}
\end{center}
\vskip -0.3in
\end{table}

==> s-acknowledgment.tex <==
\section{Acknowledgements}
\label{acknowledgements}
We would like to thank the entire OffWorld team for their enthusiastic support of this work. Special thanks to Ashish Kumar for help in the setup of experiments and for many hours of fruitful discussions.
